NeuroCounterfactuals: Beyond Minimal-Edit Counterfactuals for Richer Data Augmentation

While counterfactual data augmentation offers a promising step towards robust generalization in natural language processing, producing a set of counterfactuals that offer valuable inductive bias for models remains a challenge. Most existing approaches for producing counterfactuals, manual or automated, rely on small perturbations via minimal edits, resulting in simplistic changes. We introduce NeuroCounterfactuals, designed as loose counterfactuals, allowing for larger edits which result in naturalistic generations containing linguistic diversity, while still bearing similarity to the original document. Our novel generative approach bridges the benefits of constrained decoding, with those of language model adaptation for sentiment steering. Training data augmentation with our generations results in both in-domain and out-of-domain improvements for sentiment classification, outperforming even manually curated counterfactuals, under select settings. We further present detailed analyses to show the advantages of NeuroCounterfactuals over approaches involving simple, minimal edits.

==> tables/app-tab-self-bleu.tex <==
\begin{table}[ht]
\centering
\small
% \resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l c c c c}
\toprule
\textbf{Source of CFs}&  \textbf{Self-BLEU} \\
\midrule
% Human \cite{gardner2020evaluating} & 0.8370 & 0.6982 & 121 & 0.7376\\
\HandPencilLeft~\citealp{kaushik2019learning}  & 0.7668  \\
\midrule
\citealp{yang2021exploring}  & 0.7307 \\
\citealp{wang2021robustness}  & 0.7081 \\
\ncfneu  & 0.7795  \\
$\quad$ w/ concept-altered  & 0.7546  \\
\ncfuni  & 0.8366 & \\
$\quad$ w/o constraints  & 0.7957  \\
\bottomrule
\end{tabular}
% }
\caption{Self-BLEU ($n$-gram$ =2$) scores between CFs from various sources and the original.}
\label{tab:self-bleu}
\end{table}

==> tables/arxived/tab_ctfVsC.tex <==
\begin{table*}[ht]
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l | l | c c c c}
\hline
\textbf{Counterfactuals} & \textbf{Training Data (IMDB-S)} & \textbf{IMDB-S CTF} & \textbf{Amazon} & \textbf{Twitter} & \textbf{Yelp} \\
\hline
Auto-generated & Orig. \& CAD (\textsc{NeuroLogic} Contrast Set) & \textbf{0.772} & 0.901 & 0.757 & \textbf{0.940}\\
Auto-generated & Orig. \& CAD (\textsc{NeuroLogic} Counterfactuals) & 0.751 & \textbf{0.911} & \textbf{0.760} & 0.945\\
\hline
\end{tabular}}
\caption{Comparison of test set accuracy for RoBERTa-base trained with contrast sets or only counterfactuals generated by our approach}
\label{tab:ctfVsC}
\end{table*}


==> tables/arxived/tab_idTest.tex <==
\begin{table*}[ht]
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l | l | c c}
\hline
\textbf{Counterfactuals} & \textbf{Training Data (IMDB-S)} & \textbf{Original Test} & \textbf{Counterfactuals Test} \\
\hline
Not used & Orig. & 0.791 & 0.733 \\
\hline
Auto-generated & Orig. \& CAD (\textsc{NeuroLogic}) & 0.794 & \textbf{0.772}\\
Auto-generated & Orig. \& CAD \cite{wang2021robustness} & 0.799 & 0.764 \\
Auto-generated & Orig. \& CAD \cite{yang2021exploring} & \textbf{0.800} & 0.756 \\
\hline
Human & Orig. \& CAD \cite{kaushik2019learning} & 0.775 & 0.835 \\
\hline
\end{tabular}}
\caption{IMDB-S original \& counterfactuals test set accuracy of RoBERTa-base trained with the IMDB-S dataset and various sets of counterfactuals}
\label{tab:idTest}
\end{table*}

==> tables/arxived/tab_oodTest.tex <==
\begin{table*}[ht]
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l | l | c c c}
\hline
\textbf{Counterfactuals} & \textbf{Training Data (IMDB-S)} & \textbf{Amazon} & \textbf{Twitter} & \textbf{Yelp} \\
\hline
Not used & Orig. & 0.841 & 0.737 & 0.914\\
\hline
Auto-generated & Orig. \& CAD (\textsc{NeuroLogic}) & \textbf{0.921} & \textbf{0.774} & \textbf{0.942}\\
Auto-generated & Orig. \& CAD \cite{wang2021robustness} & 0.848 & 0.652 & 0.923\\
Auto-generated & Orig. \& CAD \cite{yang2021exploring} & 0.855 & 0.668 & 0.810\\
\hline
Human-generated & Orig. \& CAD \cite{kaushik2019learning} & 0.920 & 0.696 & 0.933\\
\hline
\end{tabular}}
\caption{Out-of-domain test set accuracy of RoBERTa-base trained with the IMDB-S dataset and various sets of counterfactuals.
\swabha{Could potentially be combined with Table~\ref{tab:idTest}}}
\label{tab:oodTest}
\end{table*}

==> tables/tab-noConstraintAblation.tex <==
\begin{table*}[ht]
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l  r c c c c c c}
\toprule
\textbf{Counterfactuals Source}& $|D_{train}|$ & \textbf{IMDB-S Test} & \textbf{IMDB-S CTF} & \textbf{SST-2} & \textbf{Twitter} & \textbf{Yelp} & \textbf{Amazon} \\
\midrule
\ncfs  & 9,130 & $80.34_{0.53}$ & $\mathbf{76.41}_{0.83}$ & $\mathbf{91.57}_{0.65}$ & $\mathbf{78.66}_{1.59}$ & $\mathbf{95.02}_{0.36}$ & $\mathbf{91.39}_{0.82}$\\
$\quad$ w/o constraints & 9,130 & $\mathbf{80.41}_{0.46}$ & $75.30_{0.90}$ & $90.54_{0.92}$ & $78.51_{1.51}$ & $94.64_{0.79}$ & $90.34_{1.09}$ \\
\midrule[0.03em]
\ncfs & 10,376 & $80.28_{0.37}$ & $\mathbf{76.92}_{0.81}$ & $\mathbf{92.16}_{0.45}$ & $\mathbf{78.85}_{1.55}$ & $\mathbf{95.10}_{0.41}$ & $\mathbf{91.96}_{0.70}$\\
$\quad$ w/o constraints & 10,376 & $\mathbf{80.49}_{0.44}$ & $75.05_{0.91}$ & $90.54_{0.69}$ & $78.65_{1.51}$ & $94.39_{0.69}$ & $90.01_{1.02}$ \\
\midrule
\ncfs & 15,437 & $79.07_{0.47}$ & $\mathbf{77.92}_{0.73}$ & $\mathbf{92.68}_{0.47}$ & $\mathbf{77.89}_{1.20}$ & $\mathbf{94.99}_{0.24}$ & $\mathbf{92.33}_{0.51}$ \\
$\quad$ w/o constraints & 16,313 & $\mathbf{80.20}_{0.42}$ & $74.85_{0.77}$ & $90.37_{0.75}$ & $77.76_{1.59}$ & $93.19_{1.99}$ & $89.10_{1.48}$ \\
\bottomrule
\end{tabular}}
\caption{Comparison of mean test set accuracy of RoBERTa-base trained on CAD generated with constraint-based decoding (\neurologic) and without constraints (sentiment expert).
\swabha{these results are best presented as a graph}}
\label{tab:noConstraintAblation}
\end{table*}
